QuReed

We present QuReed, an open-source quantum simulation framework designed to bridge gaps between quantum theory, experimental community and engineering. With Quantum Mechanics maturing and holding significant potential beyond quantum computing, the need for physically accurate simulations becomes critical. QuReed offers peer-reviewed simulation models, providing researchers and engineers with reliable tools for exploring quantum communication protocols and applications. By facilitating cross-talk between theory and experiments, QuReed aims to accelerate progress in the field and unlock the transformative power of quantum mechanics in the communications industry. Its user-friendly Python interface and comprehensive documentation ensure widespread accessibility and usability, making QuReed a valuable resource for advancing quantum communication technologies.

==> paper/v1_01_introduction.tex <==

\section{Introduction}
Quantum Mechanics is a mature theory and with all of the advances in the theory, we are on the brink of bringing the theory to the industry. The field of quantum computing is already flowering, but quantum mechanic theory has much more to offer than only computing. It is bound to change how we perceive different aspects of communication. With it one can enable physically secure communication through various protocols, further it can enable higher communication rates with new receiver designs and lastly, it can enable new networked applications from quantum byzantine tolerance to quantum leader election with many more applications and protocols to come as the industry matures. 

With theory vastly preceding the experimentalists and engineers we need to put current knowledge effectively to work. To bring the quantum theory to communications industries the knowledge need to be disseminated from theory to experiments and finally to the field of engineering. Currently the process of discovery relies on two methods experiments and simulations, which are both academic disciplines in their own right. Experiments require  a lot of expertise and more importantly capital commitment without the guarantee of a discovery applicable to the industry. The experiments never the less crucial in the advancing of the field. Another method, simulations, is widely available through many quantum optical simulators. While the simulators are usually very accessible, they lack the crucial component: \textbf{physical realism}.

The lack of physical realism makes the field of quantum simulations and the filed of quantum optical experiments two distinct disciplines with little cross talk. Such cross talk would result in cross pollination of ideas and it would have the potential to move current barriers of the communications industry. For this reason we present open sourced quantum simulation framework: \textbf{QuaSi}, the main objective of which is giving end users access to physically accurate simulations, with peer reviewed simulation models. The framework features a easy to use collection of components, which are peer reviewed to ensure not only accuracy but also correctness. The framework takes end user into account by providing easy to use Python interface with thorough documentation. The scope of the simulation is limited by the computational power at hand.

==> paper/v1_02_state_of_the_art.tex <==
\section{State of the art}

==> paper/v1_03_architecture.tex <==
\section{Architecture}
The \textit{QuaSi} platform is a platform aiming to provide a wast verified library of compatible modules, which simulate the action of quantum hardware.


This section describes the inner workings of the QuaSi framework. First we describe the simulation engine, together with the in-depth explanation of the simulation backends developed for the sole purpose of this framework. Then the concept of a device is presented, together with the concept of the signals. In the last section we touch upon the graphical user interface.





\subsection{The Simulation Database}
The QuaSi offers a freely available component database, which can be used to simulate the

Contributor should:
\begin{itemize}
    \item Correctly specify the operating ranges, in particular provide description of component:
        \begin{itemize}
            \item \emph{in time} (what is the I/O relation in time)
            \item \emph{in space} (including the port sizes)
            \item \emph{in frequency} (operating frequency ranges)
        \end{itemize}
    \item Provide Hamiltonian
    \item Provide In- and Output Hilbert Spaces
    \item Provide numerical evidence the component does simulate the Hardware accurately
    \item Provide the dependence of simulation accuracy on Hilbert space sizes and on signal durations
\end{itemize}

Reviewer should:
\begin{itemize}
    \item make sure that the component is tested with the simulation
    \item the results should reflect the stated results in the contributing paper
    \item the simulation which reflects the paper should not produce warnings (all used components must be used with compatible components)
\end{itemize}

User should:
\begin{itemize}
    \item be notified in case they are using a component outside of the operating range.
    \item have a way of browsing large library of components.
\end{itemize}

% Database

\subsection{The Simulation Engine}

% Contributions should be language agnostic
% QuaSi supplies the 'glue' which connects the components together
% 

The \textit{QuaSi} tool aims to provide a user with a rich library of accurate and simulatable hardware components. All of the already implemented components and future components should rely on the simulation kernel provided by the \textit{QuaSi} framework. QuaSi relies on various backends, where each backends supports different type of quantum simulation.

QuaSi implements it's own backend for simulations of number states - Fock backend as well as backend which supports Hamiltonian simulation. Other backends include QuTIP\cite{johansson2012qutip} and Qiskit\cite{Qiskit}. The aim is for all of the implemented components to use any of the given backends, however the authors realize this might not also be possible. Taking this into account the \textit{QuaSi} offers the user to simulate with any method, given the selected components implement the required functionalities. When using a \gls{gui}, user can in advance filter the components, that have desired simulation method implemented.

In the following sections we describe the implemented backends: Fock backend and Hamiltonian backend.

\subsubsection{Fock Backend}
In quantum mechanics (QM), particles can be categorized as \textit{fermionic} or \textit{bosonic}. A big portion of the literature about QC and the industry focuses on the formalism of the two-level system denoted by the $\ket{0}$ and $\ket{1}$ states and can be efficiently described by a complex Hilbert space denoted by $\mathcal{H}$ spanning all the possible combinations of these states. It's also called the discrete model of QC. The physical realization for such a system would be Superconducting qubits or Ion-Trapped qubits, however other hardware implementations are also considered like $\cdots$. With an appropriate set of operators or gates and enough number of qubits, this formalism can simulate any classical function.\\

On the other hand, quantum computers that use bosonic particles such as \textit{photons} to simulate a quantum process or to perform a logical operation, do have a higher degree of freedom in terms of the number of particles that can be within a single state and the fact that we can have a system that is composed of different states and each state has different $N$ particles.
To explain this visually, let's consider a Harmonic Oscillator (HO) with mass $m$ moving inside a quadratic potential energy function of displacement
\begin{equation} \label{v(x)}
    V(x)=\frac{1}{2}kx^2,
\end{equation}
its Schrödinger equation will be
\begin{equation}\label{QHO}
    E \psi(x) = -\frac{\hbar^{2}}{2m} \frac{d^{2}}{d x^{2}}\psi(x) + \frac{1}{2} kx^2 \psi(x).
\end{equation}
The eigenstates of equation \eqref{QHO} can be written in terms of the Hermite polynomials as
\begin{equation}\label{eigenstate}
    \psi_n(x) = \mathcal{N}_n  H_n(x) e^{-x^2/2},
\end{equation}
where $\mathcal{N}_n = (\sqrt{\pi} 2^n n!)^{-1/2}$ is a normalization factor, $H_n$ is the Hermite polynomial of order $n$, and $n \in \mathbb{N}$ is the quantum number. The eigenvalues can be computed as a function of $n$
\begin{equation}\label{eigenvalues of HO}
    E_n= \hbar \omega \Big (n+\frac{1}{2}\Big),
    \end{equation}
where $\omega$ is the angular frequency that is dependent on $k$ and $m$. Figure \ref{graphic:QHO}, depicts the different energy levels and the associated quanta particles in each level for a single quantum HO. In this manner we can describe a single quantum HO as an equivalent to a single qubit. From such analogy, it's obvious that there are much more degrees of freedom in the photonic system than the qubit one has. If there are multiple disjoint quantum HOs for a system, then a special Hilbert space must be introduced to efficiently describe the quantum system.
\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.8]{paper/assets/QHO.jpg}
	\caption{Different energy levels of a Quantum HO. By setting $\hbar$ and $\omega$ to be $1$, equation \eqref{eigenvalues of HO} will be $(n+0.5)$. This is the reason for the shifted energy level at $n=0$. It's also obvious that each energy level is equally spaced.}
	\label{graphic:QHO}
\end{figure}

Named after Vladimir A. Fock, the Fock space was introduced in 1932. For a Hilbert space $\mathcal{H}$ that contains a single particle or a quantum state that could be either $\ket{0}$ or $\ket{1}$, the tensor product $\mathcal{H}\otimes\mathcal{H}$ will be the space that fully characterizes the quantum states of the same two particles within it. One can generalize this to $\mathcal{H}^{\otimes N}=\otimes_{k=1}%
^{N}\mathcal{H}_{k}$ for $n$ particles. Since we focus on photonic QC, we shall focus on the bosonic Fock space which is also called the symmetrized tensor product of Hilbert spaces.

A single mode state can be decomposed into the Fock basis as follows:
\[
\ket{\psi} = \sum_n c_n \ket{n},
\]
if there exists a unique integer $m$ such that
\[
\begin{cases}c_n=1& n=m\\c_n=0&n\neq
m\end{cases},
\]
then the single mode is simply a Fock state or  $n$ photon state.
When working with an $N$-mode density matrix in the Fock basis,
\[
\rho = \sum_{n_1}\cdots\sum_{n_N} c_{n_1,\cdots,n_N}\ket{n_1,\cdots,n_N}\bra{n_1,\cdots,n_N}.
\]
We use the convention that every pair of consecutive dimensions corresponds to a subsystem; i.e.,
\[
\rho_{\underbrace{ij}_{\text{mode}~0}~\underbrace{kl}_{\text{mode}~1}~\underbrace{mn}_{\text{mode}~2}}
\]

\begin{definition}[Bosonic Fock Space]\label{define_1}
    A Bosonic Fock space is the sum of all symmetrized tensor products of a single particle Hilbert space $\mathcal{H}$
    \begin{equation}\label{fock space}
        \mathcal{F} = \bigoplus_{n=0}^{\infty} \mathcal{H}^{\odot n},
    \end{equation}
    and the  symmetrized tensor product $\odot$ is given by $\frac{1}{n!} \sum_{e \in V_n} y_{e(1)} \odot y_{e(2)} \odot \cdots \odot y_{e(n)}$ where $V_n = \{1, 2, \cdots, n\}$ is the set of permutations and $y \in \mathcal{H}$.
\end{definition}
According to definition (\ref{define_1}), if we have a quantum system of $3$ particles and $4$ modes then the state $\psi$ can be written as $|0, 1, 1, 1\rangle$, $|0, 3, 0, 0\rangle$, $|1, 0, 2, 0\rangle$, or any other combination as long as the total number of particles is equal to $3$. It's clear that the Fock space enables us to express the possibility of evaluating the expectation values of finding $N$ particles in a specific eigenstate, i.e., it becomes natural to calculate the mean photon number of a specific quantum state.\\

\subsection{Field Operators}
While developing the second quantization formalism of quantum mechanics, Paul Dirac has introduced the field operators to be used instead of wavefuncitons. There are two important field operators; the annihilation operator and its adjoint the creation operator denoted by $\hat{a}$ and $\hat{a}^\dagger$ respectively. The creation operator or the raising operator is used to increse the number of particles in a quantum system. On the other hand, the lowering operator or annihilation operator is used to remove a particle from a quantum system. These operators satisfy the bosonic commutation relations
\begin{equation}
    \lbrack\hat{a}_{i},\hat{a}_{j}^\dagger] = \hat{a}_{i} \hat{a}_{j}^\dagger - \hat{a}_{j}^\dagger \hat{a}_{i} = \delta_{ij}. \label{BCR}%
\end{equation}
The matrix representation of the creation operator is
\begin{equation}\label{creation operator matrix}
    \hat{a}^\dagger  = \begin{bmatrix}
    0 &  0 & 0 & 0 & \cdots\\ 
    \sqrt1 & 0 & 0 & 0 & \cdots\\ 
    0 & \sqrt2 & 0 & 0 & \cdots\\ 
    0 & 0 & \sqrt3 & 0 & \cdots\\
    \vdots & 0 & 0 & \ddots &  0
    \end{bmatrix}.
\end{equation}
There are also two important operators that represent the position and the momentum of a quantum system denoted by $\hat{x}$ and $\hat{p}$ respectively. They are given as
\begin{equation}\label{position and momentum operators}
    \hat{x} = \sqrt{\frac{\hbar}{2}}(\hat{a}+\hat{a}^\dagger),~~~ \hat{p} = -i \sqrt{\frac{\hbar}{2}}(\hat{a}-\hat{a}^\dagger),
\end{equation}
and they fulfil the commutation relation
\begin{equation}\label{Position and Momentum commutation rule}
    [\hat{x}_i, \hat{p}_j] = i \hbar\delta_{ij}.
\end{equation}

In a Fock space of $0$ particles or a Vacuum state denoted by $\ket{0}$, the effect of the ladder operators $\hat{a}$ and $\hat{a}^\dagger$ is
\begin{equation}\label{equation4}
    \hat{a}\left\vert 0\right\rangle =0,~~~\hat{a}\left\vert n\right\rangle
    =\sqrt{n}\left\vert n-1\right\rangle ~~\text{(for}~n\geq1\text{),}
\end{equation}
and
\begin{equation}\label{equation5}
\hat{a}^{\dagger}\left\vert n\right\rangle =\sqrt{n+1}\left\vert
n+1\right\rangle ~~\text{(for}~n\geq0\text{).}
\end{equation}
Using equation \eqref{equation5} one can create any number state or a Fock state from the Vacuum state as follows
\begin{equation}\label{equation6}
|n\rangle = \frac{(\hat{a}^\dagger)^n}{\sqrt{n!}} |0\rangle.
\end{equation}
The ladder operators can also form a hermitian operator called the \textit{Number Operator} denoted by 
\begin{equation}\label{number operator}
    \hat{n} = \hat{a}^\dagger\hat{a}.
\end{equation}

\subsection{Linear Passive Operators in the Fock Space}

There is a unitary operator called the Beamsplitter. The Beamsplitter operates on two quantum modes instead of one. It's defined as

\begin{equation}\label{beamsplitter}
    \mathcal{B}(\theta,\phi) = \exp\left(\theta (e^{i \phi}\hat{a_1} \hat{a_2}^\dagger - e^{-i \phi} \hat{a_1}^\dagger \hat{a_2}) \right).
\end{equation}
The effect on the ladder operators is given by
\begin{equation}
    \begin{split}
        \mathcal{B}^\dagger(\theta,\phi) \hat{a_1}  \mathcal{B}(\theta,\phi) &= t \hat{a_1} -r^* \hat{a_2},\\ \mathcal{B}^\dagger(\theta,\phi) \hat{a_2}  \mathcal{B}(\theta,\phi) &= t \hat{a_2} +r \hat{a_1},
    \end{split}
\end{equation}
where $t=\cos{\theta}$ is the transmittivity and here $r$ is the reflectivity amplitude and equals $e^{i\phi} \sin{\theta}$. When $\theta = \pi/4$ and $\phi = 0$ or $\phi = \pi$, the resulting operator is a 50-50 Beamsplitter. It's clear that the Beamsplitter is not an active operator since it doesn't increase the photon number in the quantum system.\\

The Rotation operator denoted by $\mathcal{R}(\phi)$ is a single mode operator that has the following transformation on the lowering operator
\begin{equation}
    \mathcal{R}(\phi) = \exp\left(i \phi \hat{a}^\dagger \hat{a}\right).
\end{equation}
It's a passive linear operator that rotates the quadrature operators depending on $\phi$.


\subsection{Coherent States}\label{cs}
    
The Glauber States or as widely known as the Coherent States (CS) of light are specific quantum states of the quantum harmonic oscillator. They can be used to describe the dynamics of a state whose ground state has been displaced from the origin. One of the main applications of CS is laser physics. CS can be generated by applying the Displacement operator \cite{book}
    \begin{equation}\label{displacement operator}
        \mathcal{D}(\alpha) = \exp(\alpha \hat{a}^\dagger - \alpha^* \hat{a})
    \end{equation}
    on a Vacuum state where $\alpha \in \mathbb{C}$ is the value of the complex displacement and $\alpha = r e^{i\theta}$ where $r \in \mathbb{R}$ is the amplitude of the displacement and $\theta \in [0, 2\pi)$ is the phase of the displacement. Setting $\alpha$ to be $0$ will be the same as the Vacuum state $|0\rangle$. In terms of the Fock space representation, the CS can be denoted as
    \begin{equation} \label{CS}
        \begin{split}
            |\alpha \rangle & = \exp(-\frac{|\alpha|^2}{2}) \exp(\alpha \hat{a}^\dagger) \exp(-\alpha^* \hat{a}) |0\rangle \\
            & = \exp(-\frac{|\alpha|^2}{2}) \exp(\alpha \hat{a}^\dagger) |0\rangle  \\
            & = \exp(-\frac{|\alpha|^2}{2}) \sum_{n=0}^{\infty} \frac{\alpha^n}{\sqrt{n!}} |0\rangle.
        \end{split}
    \end{equation}\\
    
    
The CS $|\alpha\rangle$ is a right eigenstate of the lowering operator $\hat{a}$ with an eigenvalue $\alpha$ which implies $\hat{a}|\alpha\rangle = \alpha|\alpha\rangle$. On the other hand the CS $|\alpha\rangle$ is a left eigenstate of the raising operator $\hat{a}^\dagger$ which can be denoted by $\langle\alpha|\hat{a}^\dagger = \alpha^*\langle\alpha|$. The former two results can be summarized as
    \begin{equation}\label{cs_eigen}
        \mathcal{D}^\dagger(\alpha) \hat{a} \mathcal{D}(\alpha) = \hat{a} + \alpha \boldsymbol{I},
    \end{equation}
    \begin{equation}\label{cs_eigen_left}
        \mathcal{D}^\dagger(\alpha) \hat{a}^\dagger \mathcal{D}(\alpha) = \hat{a}^\dagger + \alpha^* \boldsymbol{I}.
    \end{equation}
The same can be shown for the quadrature operators $\hat{x}$ and $\hat{p}$
    \begin{equation}
        \begin{split}
        \mathcal{D}^\dagger(\alpha) \hat{x} \mathcal{D}(\alpha) = \hat{x} +\sqrt{2 \hbar } \operatorname{Re}(\alpha) \boldsymbol{I},\\
        \mathcal{D}^\dagger(\alpha) \hat{p} \mathcal{D}(\alpha) = \hat{p} +\sqrt{2 \hbar } \operatorname{Im}(\alpha) \boldsymbol{I}.
        \end{split}
    \end{equation}
Using equations \eqref{cs_eigen} and \eqref{cs_eigen_left}, the expectation value of the number operator $\hat{n}$ can be found as
    \begin{equation}\label{mean photon number coherent}
        \begin{split}
            \bra{\alpha}\hat{n}\ket{\alpha} &= \bra{0}\mathcal{D}^\dagger(\alpha)\hat{n}\mathcal{D}(\alpha)\ket{0}\\
            &=\bra{0} (\hat{a}^\dagger + \alpha^*)(\hat{a} + \alpha)\ket{0}\\
            &=|\alpha|^2
        \end{split}
    \end{equation}
    The inner product $\braket{.,.}$ between two CSs $\ket{\alpha}$ and $\ket{\beta}$ is given as
    \begin{equation}
        \braket{\alpha,\beta} = \exp(-\frac{|\alpha|^2}{2})\exp(-\frac{|\beta|^2}{2}) \sum_{n=0}^{\infty} \sum_{m=0}^{\infty} \frac{\beta^n}{\sqrt{n!}} \frac{(\alpha^*)^m}{\sqrt{m!}},
    \end{equation}
    which can be rewritten in a compact form as
    \begin{equation} \label{cs_inner}
        |\braket{\alpha,\beta}|^2 = \exp(-|\alpha - \beta|^2).
    \end{equation}
    It's clear that equation (\ref{cs_inner}) will evaluate to $1$ if and only if $\alpha = \beta$. In case of having a large difference between the displacement values, equation (\ref{cs_inner}) can be approximated to $0$.
    
\subsection{Squeezed States}
    Discovered by Earle Hesse Kennard, Squeezed light states are a type of non-classical states of light that allow to have low uncertainty or noise below the standard quantum limit in one of the quadrature operators while the other quadrature has an increased uncertainty. Thus, a squeezing operation obeys the Heisenberg principle and introduces a new prospective to the typical CS characteristics that can be considered as a classical Gaussian wave-packet. It's mostly used in Quantum Sensing, Radiometry, and Entanglement-based quantum key distribution. The squeezing operator $S(z)$ is \cite{book}
    \begin{equation}\label{squeezing operator}
         \mathcal{S}(z) =\exp\left(\frac{1}{2}\left(z^* \hat{a}^2-z \hat{a}^{\dagger^2}\right) \right),
    \end{equation}
    where $z = r e^{i\phi}$, with $r \in [0, \infty)$ and $\phi \in [0, 2\pi)$.
    A Squeezed state is generated by applying the squeezing operator to a Vacuum state
    \begin{equation}\label{squeezed state representation}
        \begin{split}
            \ket{z} &= \mathcal{S}(z)\ket{0}\\
            & = \sqrt{\sech r} \sum_{n=0}^{\infty} \frac{\sqrt{(2n)!}}{2^n n!} (-e^{i\phi} \tanh r)^n \ket{2n}.
        \end{split}
    \end{equation}
    
    
    The effect of the squeezing operator on the ladder operators is
    \begin{equation}
        \begin{split}
            \mathcal{S}^\dagger(z) \hat{a} \mathcal{S}(z) &= \hat{a} \cosh(r) -\hat{a}^\dagger e^{i \phi} \sinh (r),\\  \mathcal{S}^\dagger(z) \hat{a}^\dagger \mathcal{S}(z) &= \hat{a}^\dagger
        \cosh(r) -\hat{a} e^{-i \phi} \sinh(r),
        \end{split}
    \end{equation}
    and the transformation on the quadrature operators is given by
    \begin{equation}\label{squeezing operator effect}
        \mathcal{S}^\dagger(z) \hat{x}_{\phi} \mathcal{S}(z) = e^{-r}\hat{x}_{\phi}, ~~~ \mathcal{S}^\dagger(z) \hat{p}_{\phi} \mathcal{S}(z) = e^{r}\hat{p}_{\phi}
    \end{equation}
    Using the above transformation, one can compute the mean photon number of a Squeezed state as
    \begin{equation} \label{mu of photon of squeezed}
        \begin{split}
            \bra{z}\hat{n}\ket{z} &= \bra{0}\mathcal{S}^\dagger(z)\hat{a}^\dagger \hat{a} \mathcal{S}(z)\ket{0}\\
            & =\bra{0} \left(\hat{a}^\dagger \cosh(r) - \hat{a} e^{-i\phi}\sinh(r)\right) 
            \left(\hat{a}\cosh(r) - \hat{a}^\dagger e^{i\phi}\sinh(r)\right)\ket{0}\\
            & = \sinh{r}^2,
        \end{split}
    \end{equation}
    and the inner product between two Squeezed states can be calculated as
    \begin{equation}
    \label{squeezed state inner product}
        \braket{z_1,z_2} = \frac{1}{\sqrt{\cosh{r_1}\cosh{r_2} - e^{i(\phi_1 - \phi_2)}\sinh{r_1}\sinh{r_2}}}.
    \end{equation}

\subsection{Displaced Squeezed States}

Combining the action of the Squeezing (\ref{squeezing operator}) and the Displacement operators (\ref{displacement operator}), a Displaced Squeezed State (DSS) which is denoted by $\ket{\alpha, z}$  can be obtained by squeezing a Vacuum state and then displacing it as
\begin{equation}\label{displaced squeezed}
\ket{\alpha, z} = \mathcal{D}(\alpha)\mathcal{S}(z)\ket{0},
\end{equation}
and by using equations \eqref{displacement operator}, \eqref{CS}, \eqref{squeezing operator}, and \eqref{squeezed state representation}, the DSS can be expressed in terms of the Fock basis \cite{book}
\begin{equation}
    \label{DSN}
    \ket{\alpha, z} = e^{-\frac{1}{2}|\alpha|^2-\frac{1}{2}{\alpha^*}^2 e^{i\phi}\tanh{(r)}} \sum_{n=0}^\infty\frac{\left[\frac{1}{2}e^{i\phi}\tanh(r)\right]^{n/2}}{\sqrt{n!\cosh(r)}} H_n\left[ \frac{\alpha\cosh(r)+\alpha^*e^{i\phi}\sinh(r)}{\sqrt{e^{i\phi}\sinh(2r)}} \right]\ket{n},
\end{equation}
since the transformation on the ladder operators is given by
\begin{equation}\label{ladder operator transformation from displaced squeezed state}
    \begin{split}
        \mathcal{D}(\alpha)\mathcal{S}(z) \hat{a} \mathcal{D}^\dagger(\alpha)\mathcal{S}^\dagger(z) & = (\hat{a} - \alpha)\cosh{r} + (\hat{a}^\dagger - \alpha^*)e^{i\phi}\sinh{r}, \\
        \mathcal{D}(\alpha)\mathcal{S}(z) \hat{a}^\dagger \mathcal{D}^\dagger(\alpha)\mathcal{S}^\dagger(z) & = (\hat{a}^\dagger - \alpha^*)\cosh{r} + (\hat{a} - \alpha) e^{-i\phi}\sinh{r}.
    \end{split}
\end{equation}
Similarly, the mean photon number of the DSS can be obtained by a unitary transformation as in equations \eqref{mean photon number coherent} and \eqref{mu of photon of squeezed}
\begin{equation}
    \label{mean photon DSS}
    \bra{\alpha, z}\hat{n}\ket{\alpha, z} = \sinh^2{r} + \vert\alpha\vert^2.
\end{equation}

The inner product between two DSSs is \cite{inner_ds}
\begin{equation}\label{inner displaced squeezed}
    \bra{\alpha_1, z_1}\alpha_2, z_2\rangle = \beta_{21}^{-\frac{1}{2}} \exp\left\{\frac{\gamma_{21} \gamma_{12}^*}{2\beta_{21}} +  \frac{(\alpha_2 \alpha_1^* - \alpha_2^*\alpha_1)}{2} \right\},
\end{equation}
where $\beta_{21} = \cosh{r_2}\cosh{r_1}  - e^{i(\phi_2 - \phi_1)}\sinh{r_2}\sinh{r_1}$ and $\gamma_{21} = (\alpha_2 - \alpha_1)\cosh{r_2} + e^{i\phi_2}(\alpha_2^* - \alpha_1^*)\sinh{r_2}$. It's obvious that when $\alpha=0$, the right-hand side will become identical to equation \eqref{squeezed state inner product} and when $z = 0$ the inner product will  be similar to equation \eqref{cs_inner}. The squeezing part does play an important role in discriminating two quantum states since the CS are not orthogonal from their definition in section \ref{cs}.\\

\subsection{Non-Gaussian States}

From a computational point of view, a generalized DSS can be fully characterized by its Gaussian formalism with the Quadrature operators ordered in a vectorial form and a Covariance matrix that describes the correlations between different modes in a quantum system. This means that a DSS can be efficiently simulated by a classical computer. In Fact, any quadratic Hamiltonian can be decomposed into Squeezing, Displacement, Rotation, and Beamsplitter operators.\\

On the other hand, the Fock state or the Number state is not a Gaussian state. Moreover, higher-order Hamiltonians are required for a universal model of computation. This means that there should be an operator that contains higher-order terms. For instance, the Cubic Phase operator is denoted by $\mathcal{V}(\Gamma) = \exp\left\{i \frac{\Gamma}{3 \hbar} \hat{x}^3\right\}$ where $\Gamma \in \mathbb{R}$. It transforms the lowering operator by the following formula $\mathcal{V}^\dagger(\Gamma) \hat{a} \mathcal{V}(\Gamma) = \hat{a} + i\frac{\Gamma}{2\sqrt{2/\hbar}} (\hat{a} +\hat{a}^\dagger)^2
$. Utilizing such an operator along with the other linear operators will allow us to decompose higher-order Hamiltonians and simulate them efficiently on a photonic quantum computer \cite{Lloyd_1999}.\\
\begin{figure}[!ht]
\centering
\subfigure[Vacuum State]{\label{fig:vac}{\includegraphics[width=0.4\textwidth]{paper/assets/cubic_wig-min.jpg}}}\hfill
\subfigure[Fock State of $\ket{1}$]{\label{fig:fock_1}{\includegraphics[width=0.4\textwidth]{paper/assets/fock_wig-min.jpg}}}
\label{fig:fock}
\vfill
\subfigure[DSS]{\label{fig:dss}{\includegraphics[width=0.4\textwidth]{paper/assets/dis_sq_wig-min.jpg}}}
\hfill
\subfigure[A non-gaussian state denoted by $\mathcal{V}(\Gamma)\mathcal{S}(z)\ket{0}$]{\label{fig:cubic}{\includegraphics[width=0.4\textwidth]{paper/assets/cubic_wig-min.jpg}}}
\caption{The Wigner function distributions for different Fock states.}
\label{fig:subfigures}
\end{figure}
To visually express the quantumness arising from non-gaussian operators and to also study different Fock states, the Wigner Function or the quasi-probability distribution is a systematic method to describe them in terms of the phase-space formalism. Furthermore, the Wigner function is real-valued and encompasses the whole quadrature field operators. It can be calculated using a pure or a mixed state. The Wigner function is defined as
\begin{equation}\label{wigner}
    W(x,p) = \frac{1}{\pi \hbar} \int_{-\infty}^{\infty}
\psi^*(x+y)\psi(x-y)
e^{2i p y / \hbar} dy
\end{equation}
From figure \ref{fig:subfigures} and equation \eqref{wigner}, we can detect a non-gaussian state by looking at the negative part of the quasi-probability distribution. As expected, Squeezed, Displaced, Displaced Squeezed, and Vacuum states have a positive real-valued outcome. However, any Fock state that has a non-gaussian operation like Cubic phase or Number states, dose have a negative real-valued outcome from the Wigner function.



\subsubsection{Hamiltonian Backend}





\subsection{Devices}
A \emph{Device} abstracts the actions of one specific quantum device. Each device inherits structure and actions from a device archetype. This approach preserves congruence. This method also allows for devices, implemented by different authors, to be used together. There are also mechanisms in place to enforce such a structure. 

Based on the archetype all devices need to implement a few methods and interfaces. 


A device implements different methods, which simulate the actions of the device in the experiment. Depending on the understanding of the device's actions different simulatable actions are implemented. These implementable actions are not limited to the Python programming language. Using a wrapper, one can implement these actions in various programming language.

Devices can receive and emit signals through ports. When a device is defined as a python class, it also defines ports for the devices. The execution of a simulation method is conditioned on the signal arrival. It is important to differentiate between the simulation time and simulated time. 

Although the framework's main goal is physical accuracy, it has implemented a set of ideal devices. With ideal devices, one can compare the effect of physical realism on the experiment. The set of ideal devices includes: fiber, single photon source, beam-splitter, single photon detector. 



\begin{minted}{Python}
class Device(ABC):
    def __init__(self):
        raise NotImplementedException
\end{minted}

\subsubsection{Signals}
As in experimentation setup, the devices are connected and these connections are represented by so called Signals. The signal represent any type of signal, either classical or quantum, which can be produced or consumed by a device. 

\subsection{Simulations}


==> paper/v1_04_example_simulations.tex <==
\section{Usage Example}

To showcase the benefits of the \textbf{QuaSi} framework we present a few potential workflows from the viewpoint of user who wishes to use implemented devices only, as well as from the viewpoint of user, who wants to implement their own device, which is one of the prerequisits of contributing a device to the \textbf{QuaSi} project.

==> paper/v1_05_ideal_components.tex <==
\section{Ideal Components}

To increase the initial usefulness of the \textit{QuaSi} platform, some ideal component descriptions are already present. In this section we give a detailed description of the components from all required perspectives. Included ideal components are also available in the GUI version of the \textit{QuaSi}.

\subsection{Ideal Single Photon Source}
Ideal single photon source is a useful device active optical device, with its origins in the \textit{faint} laser\cite{al2008characterization}. There are other realizations such as X and X CITE. However they are far from ideal EXPLAIN.

In our work we define a single photon source as a source which can produce a photon at any chosen wavelength on command with 100\% efficiency.



\subsection{Ideal Coherent Light Source}

\subsection{Ideal Phase Shifter}

\subsection{Ideal 50:50 Beam Splitter}

Beam splitter\cite{prasad1987quantum} is an essential and well understood\cite{laloe2012quantum} component used by experimentalists. Beam splitter was for example used in the famous LIGO experiment \cite{fricke2012dc}. Other well known experiments include EPR experiment\cite{rarity1990experimental} as well as Hong-Ou-Mandel\cite{ou1987relation} experiment \cite{bouchard2020two}. This list is not exhaustive, but it paints the picture of importance of beam splitter as the tool of choice for experimentalists.

\noindent
\begin{minipage}{0.55\textwidth}
The action of a beam splitter is governed by an input-output relation. In two-mode beam splitter (as in this example) the input-output relation is expressed in terms of annihilation and creation operators associated with the incoming and outgoing modes of the beam splitter. Figure \ref{fig:beamsplitter} pictures a common diagram representation of the beam splitter with four ports. 
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}%
\begin{figure}[H]
    \centering
    \begin{tikzpicture}
        \draw[blue, fill=blue!20, rotate=45, rounded corners=2pt] (0,0) rectangle (1,1);
        \draw[blue, thick] (-0.675,0.707) -- (0.675,0.707);
        \draw [-{Latex[length=3mm]}, thick] (-1,1.707) -> (0,0.707) node[pos=0.2, below left] {$\hat a$};
        \draw [-{Latex[length=3mm]}, thick] (-1,-0.292) -> (0,0.707) node[pos=0.2, above left] {$\hat a$};
        \draw [-{Latex[length=3mm]}, thick] (0,0.707) -> (1,1.707) node[pos=0.8, below right] {$\hat a$};
        \draw [-{Latex[length=3mm]}, thick] (0,0.707) -> (1,-0.292) node[pos=0.8, above right] {$\hat a$};
    \end{tikzpicture}
    \caption{Schematic description of beam-splitter.}
    \label{fig:beamsplitter}
\end{figure}
\end{minipage}

\subsubsection{Fock Picture}

In the Fock Picture, the state consumed by the beam splitter as well as the state produced by it is a number state $\ket{n}$.

\begin{minted}{Python}
from quasi.components import Device

class IdealBeamSplitter(Device):
    def __init__(self):
        raise NotImplementedException
\end{minted}

\subsubsection{Hamiltonian Picture}

The Hamiltonian for such a system is trivial.



\subsection{Ideal Single Photon Detector}


\section{Investigative Components}
Besides the ideal components, QuaSi ships with investigative components. These components, do not represent any actual device. They however, offer a easy way of investigating specific properties of the simulation. They range from devices, which investigate various features of the quantum state at specific point in the experiment from modifying type of simulation carried out, to collect specific parameters of the configuration. In this section we list the existing investigative components which ship with the current version of QuaSi.


==> paper/v1_06_benchmarking.tex <==
\section{Benchmarking}
Benchmarking is an important process in software validation. In this section we
benchmark the quasi in terms of physical accuracy, computational performance as
well as user and developer friendliness.


==> paper/v1_100_meeting_notes.tex <==
\section{Meeting Notes}

\subsection{Stefan Krastanov}
\subsubsection{27.10.2023}
\begin{itemize}
    \item Working on protocols for nv centers
    \item Debugging Tooling simulator
    \item Want to build a cluster state with bigger simulation
    \item Google Sheet document for tracking progress
    \item Database of states
    \item Database of hardware
    \item Clifford backend developed by Stefan
    \item Tensor networks $>>$ \textit{ITensor} for \textit{julia}
    \href{https://github.com/ITensor/ITensors.jl}{ITensor}
\end{itemize}


\subsection{Database Meeting}
\subsubsection{08.11.2023}
\begin{itemize}
    \item Proposed Database
    \item google form will be created to get the feedback from the partners
    \item Question: Quasi and symetrizability of an channel.
    \item How to generate 3-mode GHZ state
\end{itemize}

==> paper/v1_99_user_stories.tex <==
\newpage


\section{User Stories}
% This section is for internal purposes only
% It will not be included in the final version

\definecolor{myblueviolet}{RGB}{50,0,226}

\newcommand{\userstory}[4]{
    \begin{tcolorbox}[colback=white,colframe=myblueviolet,title={\textbf{User Story}}]
        \textbf{As} #1 \\
        \textbf{I want} #2 \\
        \textbf{So that} #3 \\
        \textbf{Acceptance Criteria:}
        \begin{itemize}[label=-, noitemsep]
            #4
        \end{itemize}
    \end{tcolorbox}
}

\textbf{User Story Template}
\userstory
    {[type of user]}
    {[an action]}
    {[a benefit/value]}
    {
        \item Criteria 1: Describe what needs to be met for the story to be considered complete.
        \item Criteria 2: Describe another condition that must be satisfied.
        \item Criteria 3: Add additional criteria as necessary.
    }
    
\subsection{Journal Submissions}
\userstory
    {Researcher}
    {publish a paper, accompanied with the simulatable models}
    {other researchers and engineers can test the hardware components as a simulatable module in their setup/use-case}
    {
        \item The tool needs to be framework/language agnostic to minimize the submission friction
    }
    
\subsection{TQSD}

\userstory
    {a Scientist, focusing on bridging the experimental physics with engineering}
    {simulate channels based on physically accurate hardware}
    {I can present the possible solutions to the engineers who can build the actual hardware}
    {
        \item Models are accurate
    }

\userstory
    {}
    {writes down the Hamiltonian}
    {customers will buy correct hardware for their needs}
    {
        \item provided software user base is large enough.
    }
    
\subsection{Kai Muller's Group}

\userstory
    {an Experimentalist}
    {to provide community with new proven, simulatable hardware models}
    {I increase the impact of my research}
    {
        \item the template must be easy to extend with limited python knowledge
        \item the actions of the API must be easy to understand (good documentation)
    }
    
\userstory
    {an Experimentalist, designing an experiment}
    {to predict the outcome of the experiment}
    {I correctly select the hardware to purchase}
    {
        \item provided hardware components need to be physically accurate,
        \item rich library of simulatable components is provided.
    }

\userstory
    {an Experimentalist, designing an experiment}
    {Simulate single component}
    {I can better understand how the component affects the experiment.}
    {
        \item provided hardware components need to be physically accurate,
        \item rich library of simulatable components is provided.
    }
    
\subsection{THORLABS}
\userstory
    {a hardware manufacturer}
    {to provide accurate simulatable models for our hardware}
    {customers will buy correct hardware for their needs}
    {
        \item provided software user base is large enough.
    }
    
    
\subsection{T-Labs}
\userstory
    {an application oriented researcher at a telco}
    {   \ \\
        1) to validate Software\\
        2) to compute/plan my experiments with high predictive accuracy
    }
    {   
        \ \\
        1) So that I can use it for prediction\\
        2) So that I waste less resources when purchasing hardware
    }
    { 
        \item ...
    }
    
\userstory
    {
    Matheus
    }
    {
    to understant the behaviour of each device, before buying
    }
    {   
    I can understand t
    }
    { 
        \item ...
    }
    
    
\subsection{CQN}

\userstory
    {A theorist working for CQN}
    {}
    {}
    {
        \item Models are accurate
    }
\subsection{Internal}

\userstory
    {Teacher}
    {present students with virtual experiment}
    {they don't need to interact with expensive devices (security)}
    {
        \item Visual interface needs to be accessible
    }

\subsection{QD-CamNetz}
\userstory
    {member of a distributed developer team}
    {to use quasi (software) to create synthetic simulations (with ideal device simulation modules)}
    {we can parallelize efforts, within the team and avoid the accrual of random delays}
    {
        \item We have realized an example (with QD-CamNetz)
    }


\subsection{Special Issue}

\userstory
    {A paper author submitting to the special issue}
    {to use the easiest (possibly quasi) tool to describe my device with simulations }
    {I can better communicate the actions of my device to the wider public}
    {
        \item Tool support my preferred quantum state formalism
        \item There is enough example data, to guide my implementation
    }
    
\userstory
    {an engineer using Special Issue submissions}
    {to tinker with the submitted components}
    {I can do rapid initial research into possible solutions for a specific problem}
    {
        \item Barrier to entry has to be extremely low
        \item I might not care a lot about performance in the initial phases
        \item I want the devices to work seamlesly
    }

\userstory
    {an author}
    {to submit a component which operates in an Gaussian Simulation Regime}
    {I can carry out \textit{efficient} simulations that are appropriate to my case}
    {
        \item Paper should be accepted if simulations are correct but.
    }
    
\userstory
    {an author}
    {to submit a component which can operate with Gaussian States and also in Fock Space regime}
    {I can test my component with components that operate in either regime}
    {}

\subsection{NEQSIS}
From the meeting on 2nd Feb 2024.

\userstory
    {an Experimentalist}
    {to present my component to the theorists and possibly engineers through my submission}
    {Theorists and engineers are more likely to cooperate with me on future work.}
    {
    \item The software should allow for simple component implementation
    \item Experimentalist don't want to deal with software design
    \item Common mental framework is used.
    }
    
\userstory
    {an experimentalist}
    {to receive input from theorist (for example about a theoretical protocol)}
    {I know how to design and optimize \textbf{experiment} and \textbf{hardware} to realize an attractive use-case.}
    {
    \item The information is passed in a common mental framework
    }


\userstory
    {a distributed group of engineers}
    {access and edit the architectural diagram}
    {I can quickly understand the architecture and the parameters of the experiment. It will help to divide and parallelize the workload.}
    {}
    

\userstory
    {a user (Student, Theoretician)}
    {Wants to simulate Hong-Ou-Mandel effect}
    {he/she can understand how the outcome differs with different delays}
    {Quasi supports temporal modes, Quasi understands notion of time, the components have time dependend action on the modes. }

==> sections/appendices/01_beamsplitter.tex <==
\subsection{Ideal Non-Polarizing Beam-Splitter}

Beam-Splitter is a rudimentary device in the optical laboratory. Here we describe the action of the ideal beam splitter as well as the implementation in \gls{sim} framework.

Suppose we have two single-photon states $\ket{\psi_a}$ and $\ket{\psi_b}$ with Gaussian temporal profiles. The temporal modes can be described by wave packets, and the temporal overlap will affect the interaction at the beam splitter.

Let the temporal profiles of the wave packets be given by a Gaussian functions:
\begin{align}
    \psi_a(t) &= \frac{1}{\sqrt{\sigma_a\sqrt{\pi}}}e^{\frac{(t-t_a)^2}{2\sigma_a^2}} e^{i\omega_a t},&
    \psi_b(t) &= \frac{1}{\sqrt{\sigma_b\sqrt{\pi}}}e^{\frac{(t-t_b)^2}{2\sigma_b^2} e^{i\omega_b t}}.
\end{align}

The values $\omega_a$ and $\omega_b$ represent the central frequencies of these two packets and times $t_a$ and $t_b$ represent central times respectively.

Now we consider standard operator for the beam splitter (as seen in \cite{makarov2022theory}, equation 17):

\begin{equation}
    \hat U_{BS} = \exp(i\phi(\hat a^\dagger_1 \hat a_2 - \hat a_1 \hat a^\dagger_2)),
\end{equation}

where we consider the action of 50:50 beam splitter, thus setting the $\phi=\pi/4$.

Now we consider possible cases for the input states. If only one photon enters beam splitter at port A, then the output can simply be computed as:

\begin{align}
    \begin{split}
        \ket{\psi_{out}} = \hat U_{BS} \ket{1}_{A, t_0}\ket{0}_{A, t_0} = ()
    \end{split}
\end{align}






The overlap integral between the two temporal modes is:
\begin{equation}
    \Lambda = \int_{-\infty}^{\infty}\psi_a^*(t)\psi_b(t)dt,
\end{equation}
which for given Gaussian profiles, can be computed as:
\begin{equation}
    \Lambda = \exp(-\frac{(t_a-t_b)^2}{4\sigma_a\sigma_b})\cdot \exp(-\frac{\sigma_a^2\sigma_b^2\Delta\omega^2}{\sigma_a^2 + \sigma_b^2})
\end{equation}

Now consider a beam split operator (as seen in \cite{makarov2022theory} equation 17):
\begin{align}
\hat U_{BS} &= \hat D^\dagger&
\hat D &= e^{\eta \hat L_+ - \eta^* \hat L_-},
\end{align}

with the $\hat L_-=\hat a^\dagger_1 \hat a_2$ and $\hat L_+ = \hat a_2^\dagger \hat a_1$.

Lets consider a case where the two incoming photons $\ket{1}_{a,t_1}$ and $\ket{1}_{b,t_2}$ are totally distinguishable ($\Lambda = 0 $). In practice when each of these photons interacts with the beam-splitter, the beam-splitter would assume vacuum state in the other port, which would result in the following outputs:
\begin{align}\label{eq:non_overlapping_bs}
    &\hat U_{BS} (\ket{1}_{a,t_1}\ket{0}_{b,t_1}), &
    &\hat U_{BS} (\ket{0}_{a,t_2}\ket{1}_{b,t_2}).
\end{align}

If both packets arrive at the same time, then the operation is trivial $\hat U_{BS} \ket{1}_{a,t_0}\ket{1}_{b,t_0}$. In these two cases, the central Gaussian times are not affected. It is interesting to study, what happens to packets which arrive with some delay $\tau=t_2-t_1$ such that the temporal profiles of the two packets partially overlaps ($0<\Lambda < 1$). In our model we assume that based on the overlap factor $\Lambda$, beam splitter acts on the overlapping spaces and partially on the spaces separately. In this case we need to introduce two new vacuum Fock spaces like in equation \eqref{eq:non_overlapping_bs}. In effect we need to compute an operator which acts on four Fock spaces:

\begin{equation}
    \hat U'_{BS} = \Lambda \hat U_{BS, i} +(1-\Lambda) \hat U_{BS, d},
\end{equation}

where first term represents the proportional overlapping (distinguishable) term and the second proportional non-overlapping (indistinguishable) term. Each of the two terms need to operate on four Fock spaces.

\begin{align}
    \hat U_{BS, d} &= \exp(i\phi (a_1^\dagger a_2 + a_1 a_2^\dagger)) \otimes \hat I_3 \otimes \hat I_4, \\
    \hat U_{BS, i} &= \exp(i\phi (a_1^\dagger a_3 + a_1 a_3^\dagger)) \otimes
    \exp(i\phi (a_2^\dagger a_4 + a_2 a_4^\dagger)),
\end{align}
where we consider the following auxiliary spaces $\ket{0}_3$ and $\ket{0}_4$ in a vacuum state. For a ideal 50:50 beam splitter we set $\phi=\frac{\pi}{4}$.Now we have two operators which we apply in the case of either non-overlapping photons($\hat U_{BS}$, with vacuum state), fully overlapping photons ($\hat U_{BS}$, with respective Fock state) and partially overlapping photons($\hat U'_{BS}$, with two vacuum states).



\begin{minted}{Python}
class NonPolarizingBeamSplitter(GenericDevice):
    ## ... Ports ...
    def des():
        pass
\end{minted}




==> sections/bs-theory-1.tex <==
\subsection{Ideal Beamsplitter Theory}
Define extremal states $\delta_{s,n}:=\delta_s\otimes\delta_n$, where $s$ is time and $n$ a photon number (Fock state). The Hilbert space for that is $\mathcal L_2\otimes\mathcal F$ (square integrable functions tensored with Fock space). Let $BS:\mathcal F\otimes\mathcal F\to\mathcal F\otimes\mathcal F$ be a beam-splitter. Denote by $\boxplus$ the beam-splitter acting on $\mathcal H\otimes\mathcal F\otimes\mathcal H\otimes\mathcal F$. Then
\begin{align}
	\boxplus(\delta_{s,n}\otimes\delta_{t,m})=\delta(s,t)BS(\delta_n\otimes\delta_m) + \delta(s\neq t)\delta_{s,n}\otimes\delta_{t,m}.	
\end{align}
Assume now we have not perfect broadband photon sources, but instead $\phi:=\int\delta_{s,n}\phi(s)ds$ and $\psi:=\int\delta_{t,m}\psi(t)dt$. By linearity,
\begin{align}
	\boxplus(\phi\otimes\psi) = \int\phi(s)\psi(s)\delta_s\otimes\delta_sBS(\delta_n\otimes\delta_m) + \int_{s\neq t}\phi(s)\psi(s)\delta_{s,n}\otimes\delta_{t,m}dsdt.
\end{align}
Let a measurement operator be defined via an interval $I$ and a photon number $k$ via $\Lambda_{I,k}:=\mathbbm1_I\otimes\delta_k$. Then 
\begin{align}
	\Lambda_{I,n}=\int_I\delta_i\otimes\delta_ndi.
\end{align}
Upon setting two intervals $I,J$ and photon numbers $k,l$ we may calculate the probability $p(I,J,k,l)$ of detecting $k$ photons in time slot $I$ in the left output arm and $l$ photons in time slot $J$ of the right output arm as
\begin{align}
    p(I,J,k,l) 
        &= \int_I\int_J|\langle\delta_{i,k}\otimes\delta_{j,l},\boxplus(\phi\otimes\psi)\rangle|^2didj\\
		&= \int_I\int_J|\langle\delta_{i,k}\otimes\delta_{j,l},\int\phi(s)\psi(s)\delta_s\otimes\delta_sBS(\delta_n\otimes\delta_m)ds + \int_{s\neq t}\phi(s)\psi(s)\delta_{s,n}\otimes\delta_{t,m}dsdt\rangle|^2didj\\
		&= \int_I\int_J|\delta(i,j)\phi(i)\psi(j)\delta_i\otimes\delta_itr[\delta_k\otimes\delta_lBS(\delta_n\otimes\delta_m)] + \delta(i\neq j)\phi(i)\psi(j)\delta_{i}\otimes\delta_{j}\delta(k,m)\delta(l,n)|^2didj\\
        &=\int_{I\cap J}|\phi(s)\psi(s)|^2\cdot tr[\delta_k\otimes\delta_lBS(\delta_n\otimes\delta_m)] + (1-\int_{I\cap J}|\phi(s)\psi(s)|^2)\cdot\delta(k,m)\cdot \delta(l,n).
\end{align}
Upon inserting Gaussian pulses $\phi(s)=\psi(s)=(2/\pi)^{1/4}e^{-s^2}$ and setting $I=J=(-\infty,\infty)$ we get $\phi(s)\psi(s)=(2/\pi)^{1/2}e^{-2s^2}$. Since $\int e^{-4s^2}ds=\sqrt{\pi}/2$ this implies
\begin{align}
    \int_{I\cap J}|\phi(s)\psi(s)|^2 ds 
        &= ((2/\pi)^{1/4})^4\int e^{-4s^2}ds\\
        &= (2/\pi)\sqrt{\pi}/2\\
        &= 1/\sqrt{\pi}\\
        &\approx 0.56.
\end{align}

==> sections/bs-theory-2.tex <==
\subsection{Ideal Beamsplitter Theory}
Define extremal states $\delta_{r,n}:=\delta_s\otimes\delta_n$, where $r$ is the location at time $t=0$ and $n$ a photon number (Fock state). The Hilbert space for that is $\mathcal L_2\otimes\mathcal F$ (square integrable functions tensored with Fock space). Let $BS:\mathcal F\otimes\mathcal F\to\mathcal F\otimes\mathcal F$ be a beam-splitter. Denote by $\boxplus$ the beam-splitter acting on $\mathcal H\otimes\mathcal F\otimes\mathcal H\otimes\mathcal F$. Then with $r<s<0$ and $n,m=1$ we have
\begin{align}
	\boxplus(\delta_{r,n}^{-,L}\otimes\delta_{s,m}^{-,R})(t)=
            \left\{\begin{array}{ll}\delta_{t,0}^{+,L}\otimes\delta_{t,0}^{+,R},& t+s<0\\
    \tfrac{1}{\sqrt{2}}(\delta^{+,L}_{s+t,1}\otimes\delta^{+,R}_{s+t,0} + \delta^{+,L}_{r+t,0}\otimes\delta^{+,R}_{s+t,1})  &,  \\
    \end{array}\right.
\end{align}


Assume now we have not perfect broadband photon sources, but instead $\phi:=\int\delta_{s,n}\phi(s)ds$ and $\psi:=\int\delta_{t,m}\psi(t)dt$. By linearity,
\begin{align}
	\boxplus(\phi\otimes\psi) = \int\phi(s)\psi(s)\delta_s\otimes\delta_sBS(\delta_n\otimes\delta_m) + \int_{s\neq t}\phi(s)\psi(s)\delta_{s,n}\otimes\delta_{t,m}dsdt.
\end{align}
Let a measurement operator be defined via an interval $I$ and a photon number $k$ via $\Lambda_{I,k}:=\mathbbm1_I\otimes\delta_k$. Then 
\begin{align}
	\Lambda_{I,n}=\int_I\delta_i\otimes\delta_ndi.
\end{align}
Upon setting two intervals $I,J$ and photon numbers $k,l$ we may calculate the probability $p(I,J,k,l)$ of detecting $k$ photons in time slot $I$ in the left output arm and $l$ photons in time slot $J$ of the right output arm as
\begin{align}
    p(I,J,k,l) 
        &= \int_I\int_J|\langle\delta_{i,k}\otimes\delta_{j,l},\boxplus(\phi\otimes\psi)\rangle|^2didj\\
		&= \int_I\int_J|\langle\delta_{i,k}\otimes\delta_{j,l},\int\phi(s)\psi(s)\delta_s\otimes\delta_sBS(\delta_n\otimes\delta_m)ds + \int_{s\neq t}\phi(s)\psi(s)\delta_{s,n}\otimes\delta_{t,m}dsdt\rangle|^2didj\\
		&= \int_I\int_J|\delta(i,j)\phi(i)\psi(j)\delta_i\otimes\delta_itr[\delta_k\otimes\delta_lBS(\delta_n\otimes\delta_m)] + \delta(i\neq j)\phi(i)\psi(j)\delta_{i}\otimes\delta_{j}\delta(k,m)\delta(l,n)|^2didj\\
        &=\int_{I\cap J}|\phi(s)\psi(s)|^2\cdot tr[\delta_k\otimes\delta_lBS(\delta_n\otimes\delta_m)] + (1-\int_{I\cap J}|\phi(s)\psi(s)|^2)\cdot\delta(k,m)\cdot \delta(l,n).
\end{align}
Upon inserting Gaussian pulses $\phi(s)=\psi(s)=(2/\pi)^{1/4}e^{-s^2}$ and setting $I=J=(-\infty,\infty)$ we get $\phi(s)\psi(s)=(2/\pi)^{1/2}e^{-2s^2}$. Since $\int e^{-4s^2}ds=\sqrt{\pi}/2$ this implies
\begin{align}
    \int_{I\cap J}|\phi(s)\psi(s)|^2 ds 
        &= ((2/\pi)^{1/4})^4\int e^{-4s^2}ds\\
        &= (2/\pi)\sqrt{\pi}/2\\
        &= 1/\sqrt{\pi}\\
        &\approx 0.56.
\end{align}
